TANGO: Time-Reversal Latent GraphODE for Multi-Agent Dynamical Systems

Learning complex multi-agent system dynamics from data is crucial across many domains, such as in physical simulations and material modeling. Extended from purely data-driven approaches, existing physics-informed approaches such as Hamiltonian Neural Network strictly follow energy conservation law to introduce inductive bias, making their learning more sample efficiently. However, many real-world systems do not strictly conserve energy, such as spring systems with frictions. Recognizing this, we turn our attention to a broader physical principle: Time-Reversal Symmetry, which depicts that the dynamics of a system shall remain invariant when traversed back over time. It still helps to preserve energies for conservative systems and in the meanwhile, serves as a strong inductive bias for non-conservative, reversible systems. To inject such inductive bias, in this paper, we propose a simple-yet-effective self-supervised regularization term as a soft constraint that aligns the forward and backward trajectories predicted by a continuous graph neural network-based ordinary differential equation (GraphODE). It effectively imposes time-reversal symmetry to enable more accurate model predictions across a wider range of dynamical systems under classical mechanics. In addition, we further provide theoretical analysis to show that our regularization essentially minimizes higher-order Taylor expansion terms during the ODE integration steps, which enables our model to be more noise-tolerant and even applicable to irreversible systems. Experimental results on a variety of physical systems demonstrate the effectiveness of our proposed method. Particularly, it achieves an MSE improvement of 11.5 % on a challenging chaotic triple-pendulum systems.

==> section/formulation.tex <==
\section{Problems Formulation and  Preliminaries}

We consider a dynamical system as a graph $\mathcal{G} = (\mathcal{V},\mathcal{E})$ where $\mathcal{V}$ denotes the node set of $N$ agents and $\mathcal{E}$ is the set of edges representing their physical interactions, which for simplicity we assumed to be static over time. 
We denote $\bm{X}^{t} \in \mathcal{X}$ as the feature matrix for all agents.
% and $\bm{x}_i^{t}$ as the feature vector of agent $i$ at time $t$. 
Model input consists of the trajectories over $K$ timestamps $X^{t_{1:K}}=\{\bm{X}^{t_1}, \bm{X}^{t_2}, \ldots, \bm{X}^{t_K}\}$, where the timestamps $t_1,t_2\cdots t_K$ can have non-uniform intervals and be of any continuous values. Our goal is to learn a neural simulator $f_{\theta}(\cdot) :X^{t_{1:K}}\rightarrow Y^{t_{K+1:T}}$ which predicts node dynamics $\bm{Y}^{t}\in\mathcal{Y}$ in the future. We use $\bm{y}_i^{t}$ to denote the targeted dynamic vector of agent $i$ at time $t$. 



\paragraph{GraphODE for Multi-agent Dynamical Systems.}
 Multi-agent dynamical system can be described by a series of first-order ODEs: $\dot{\bm{z}}_{i}^{t}:=\frac{d \bm{z}_{i}^{t}}{d t}=g\left(\bm{z}_{1}^{t}, \bm{z}_{2}^{t} \cdots \bm{z}_{N}^{t}\right)$. Here $\bm{z}_i^t\in\mathbb{R}^d$ denotes the latent state variable for agent $i$ at timestamp $t$ and $g$ denotes the ODE function that drives the system move forward. Traditionally, the ODE functions are hand-crafted by domain experts which is hard to generalize to other systems. Recent studies~\cite{neuralODE} propose to parameterize it with a neural network and learn it in a data-driven way. To capture the continuous interaction for multi-agent system, a series of GraphODE models~\cite{LGODE,ndcn,hope,CFGODE,wen2022social} have been proposed, which employ GNN as the ODE function and have been shown to achieve superior performance in
long-range predictions. They usually follow an encoder-processor-decoder architecture, where an encoder first computes the latent initial states $\bm{z}_{1}^{0}, 
\cdots \bm{z}_{N}^{0}$ for all agents simultaneously based on their historical observations. Then the GNN-based ODE function predicts the latent trajectories starting from the learned initial states.
Finally, a decoder extracts the predicted dynamic features based on a decoding function that takes the predicted latent states as input.


Given the initial states $\bm{z}_{1}^{0}, 
\cdots \bm{z}_{N}^{0}$ for all agents and the ODE function $g$, we can compute the latent state $\bm{z}_i^T$ at any desired time using a numerical ODE solver such as Runge-Kuttais~\citep{solver} as shown in Eqn~\ref{eq:ode}. 
\begin{equation}
    \bm{z}_{i}^{T}=\bm{z}_{i}^{0}+\int_{t=0}^{T} g\left(\bm{z}_{1}^{t}, \bm{z}_{2}^{t} \cdots \bm{z}_{N}^{t}\right) d t
    \label{eq:ode}
\end{equation}


\paragraph{Time-Reversal Symmetry.}\label{sec:time_reversal}
Let $R: \mathcal{X} \mapsto \mathcal{X}$ be a reversing operator~\cite{lamb1998time}. We consider a multi-agent dynamical system described in the matrix form of $\frac{d\boldsymbol{X}}{dt}=F(\boldsymbol{X})$ where $\boldsymbol{X} \in \mathbb{R}^{N\times d}$ is the time-varying state matrix of all agents. We omit the script of t for notation simplicity in the following. Let $\phi_\tau :\boldsymbol{X}(t) \mapsto  \phi_\tau(\boldsymbol{X}(t))=\boldsymbol{X}(t+ \tau)$ be a time evolution operator for arbitrary $t,\tau \in \mathbb{R}$, which satisfies $\phi_{\tau_1}\circ \phi_{\tau_2}=\phi_{\tau_1+\tau_2}~\text{for all } \tau_1,\tau_2 \in \mathbb{R}$\footnote{$\circ$ denotes composition}.


A dynamical system is said to follow the time-reversal symmetry if
\begin{equation}
\label{eq:def_R}
    \frac{dR(\boldsymbol{X})}{dt}=-F(R(\boldsymbol{X})),
\end{equation}
which also implies that:
\begin{equation}
    \label{eq:def_reverse}
    R \circ \phi_t=\phi_{-t} \circ R = \phi_t^{-1}\circ R
\end{equation}





%2. connection to conservative system
Time-reversal symmetry is a fundamental property in many physical systems, especially in classical and quantum mechanics. 
To inject such physical law, there is a series of works that inject the energy conservation constraints to neural ODEs~\cite{}, which achieve accurate time evolution of classical conservative systems. However, time-reversal property is a broader concept than energy conservation and can be applied to more dynamical systems. It differs from energy conservation in that, systems that are time-reversal are not necessarily conservative, but systems that are conservative must be time-reversal. Therefore, existing methods have inherent limitations in that they cannot be applied to non-conservative systems since they require the system to strictly conserve the total energy. 


%3. examples (emphasize need to be flexible), existing non-flexible baselines.
Moreover, some systems may not strictly obey the time-reversal properties due to situations such as external forces, heat transfer, and noises in observational data. 
Therefore, a desired model shall be able to learn from data whether to apply time-reversal symmetry constraint, so as to cover a wider range of real-world dynamical systems, including xxx




==> section/implementation.tex <==
\textbf{TANGO}
\par
Our implementation of TANGO follows \citep{LGODE}. We implement the initial state encoder using a 2-layer GNN with observation representation dimension of 64 across all datasets. We use ReLU for nonlinear activation. For the self-attention module, we set the output dimension to 128. The encoder's output dimension is set to 16, and we add 64 additional dimension to the output of the recognition model to stabilize the training process. The GraphODE generative model is implemented with a single-layer GNN with hidden dimension 128. To compute trajectories, we use the Runge-Kutta method from torchdiffeq python package \cite{chen2021eventfn} as the ODE solver, and a one-layer MLP as the decoder.

We implement our model in pytorch. Encoder, generative model and the decoder parameters are jointly optimized with AdamW optimizer \cite{loshchilov2017decoupled}. \ji{todo: add details} with learning rate 0.0005. Batch size for simulated datsests are set as 256.

\textbf{LatentODE}
\par
We implement the Latent ODE sequence to sequence model as specified in \cite. We use a 4-layer ODE function in the recognition ODE, and a 2-layer ODE function in the generative ODE. The recognition and generative ODE use Euler and Dopri5 as solvers \cite, respectively. The number of units per layer is 1000 in the ODE functions, and 50 in GRU update networks. The dimension of the recognition model is set to 100.  The model is trained with a learning rate of 0.001 with an exponential decay rate of 0.999 across different experiments. Note that since latentODE is a single-agent model, we compute the trajectory of each object independently when applying it to multi-agent systems.

\textbf{HODEN}
\par
To adapt HODEN, which requires full initial states of all objects, to systems with partial observations, we compute each object’s initial state via linear spline interpolation if it is missing. Following the setup in \cite, we use two 2-layer linear networks with Tanh activation in between as the ODE functions for a state and the rate of change of a state. Each network has a 1000-unit layer followed by a single unit layer.The model is trained with a learning rate of 0.00001 using a cosine scheduler.

\textbf{TRSODEN}
\par
Similar to HODEN, we compute each object’s initial state via linear spline interpolation if it is missing. As in \cite, we use a 2-layer linear network with Tanh activation in between as the ODE functions, and the Leapfrog solver \cite. The network has 1000 hidden units, and is trained with a learning rate of 0.00001 using a cosine scheduler.

==> section/method.tex <==
\section{Method}
To enforce flexible time-reversal symmetry in modeling multi-agent dynamical systems, we propose \model, a novel GraphODE framework which learns system
dynamics using neural ordinary differential equations (ODE) parameterized by a
GNN to capture the continuous interaction among agents. We achieve flexible
time-reversal constraints by introducing a novel regularization term in the loss
function, whose weight is adjustable towards different targeted systems. The overall framework is depicted in Figure~\ref{fig:framework}. We now illustrate each component in detail.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/framework.pdf}
    \caption{Overall Framework of \model}
    \label{fig:framework}
\end{figure}

\subsection{Initial State Encoder}
The initial state encoder computes the latent node initial states $\boldsymbol{z}_i^0$ for all agents simultaneously considering their mutual interaction. Specifically, it first fuses all observations into a temporal graph and conducts dynamic node representation through a spatial-temporal GNN  as in~\cite{LGODE}: 


\begin{equation}
\begin{aligned}
\boldsymbol{h}_{j\left(t\right)}^{l+1}=\boldsymbol{h}_{j\left(t\right)}^{l}+\sigma\left(\sum_{i(t') \in \mathcal{N}_{j(t)}}\alpha_{i\left(t'\right) \rightarrow j\left(t\right)}^{l}\times \boldsymbol{W}_v\hat{\boldsymbol{h}}_{i\left(t'\right)}^{l-1}\right)\\
\alpha^l_{i\left(t'\right) \rightarrow j\left(t\right)} = \left(\boldsymbol{W}_{k}\hat{\boldsymbol{h}}_{i(t')}^{l-1}\right)^{T}\left(\boldsymbol{W}_{q} \boldsymbol{h}_{j(t)}^{l-1}\right) \cdot \frac{1}{\sqrt{d}},\quad  \hat{\boldsymbol{h}}_{i\left(t'\right)}^{l-1} = \boldsymbol{h}_{i\left(t'\right)}^{l-1} + \text{TE}(t'-t)\\
\operatorname{TE}(\Delta t)_{2i}=\sin \left(\frac{\Delta t} {10000^{2 i / d}}\right),~\operatorname{TE}(\Delta t)_{2i+1}=\cos \left(\frac{\Delta t} {10000^{2 i / d}}\right),
    \end{aligned}
    \label{eq:encoder_GNN}
\end{equation}
where $||$ denotes concatenation; $\sigma(\cdot)$ is a non-linear activation function; $d$ is the dimension of node embeddings. The node representation is computed as a weighted summation over its neighbors plus residual connection where the attention score is a transformer-based~\cite{attention} dot-product of node representations by the use of value, key, query projection matrices $\boldsymbol{W}_v,\boldsymbol{W}_k,\boldsymbol{W}_q$. Here $\boldsymbol{h}_{j(t)}^l$ is the representation of agent $j$ at time $t$ in the $l$-th layer. $i(t')$ is the general index for neighbors connected by temporal edges (where $t'\neq t$) and spatial edges (where $t=t'$ and $i\neq j$). The temporal encoding ~\cite{hgt} is added to a neighborhood node representation in order to distinguish its message delivered via spatial and temporal edges. Then, we stack $L$ layers to get the final representation for each observation node: $\boldsymbol{h}_{i}^t = \boldsymbol{h}_{i\left(t\right)}^{L}$. 
Finally, we employ a self-attention mechanism to generate the sequence representation $\boldsymbol{u}_i$ for each agent as their latent initial states:
\begin{equation}
\begin{aligned}
    \bm{u}_{i}=\frac{1}{K} \sum_{t} \sigma\left(\bm{a}_{i}^T \hat{\bm{h}}_{i}^{t}\hat{\bm{h}}_{i}^{t}\right),~\bm{a}_{i}=\tanh \left(\left(\frac{1}{K} \sum_{t} \hat{\bm{h}}_{i}^{t}\right) \bm{W}_{a}\right),\\
\end{aligned}
\label{eq:encoder_sequence}
\end{equation}
 where $\boldsymbol{a}_i$ is the average of observation representations with a nonlinear transformation $\boldsymbol{W}_a$ and $\hat{\boldsymbol{h}}_{i}^{t} = \bm{h}_{i}^{t} + \text{TE}(t)$. $K$ is the number of observations for each trajectory.
Compared with recurrent models such as RNN, LSTM~\cite{LSTM}, it offers better parallelization for accelerating training speed and in the meanwhile alleviates the vanishing/exploding gradient problem brought by long sequences.


\subsection{GraphODE Generative Model and the Decoder}
Given the latent initial states, the dynamics of the whole system is determined by the ODE function $g$ which we parametrize as a GNN as in~\cite{LGODE} to capture the continuous interaction among agents. We then employ a decoder which is a two-layer Multilayer Perceptron (MLP) to predict the trajectories $\boldsymbol{\hat{y}}_i^t$ from the latent states $\boldsymbol{z}_i^t$. 

\begin{equation}
\begin{aligned}
\boldsymbol{z}_i^0,\boldsymbol{z}_i^1,\boldsymbol{z}_i^2...\boldsymbol{z}_i^T&=\text{ODEsolver}(g,[\boldsymbol{z}_1^0,\boldsymbol{z}_2^0...\boldsymbol{z}_N^0],(t_0,t_1...t_T))\\
\boldsymbol{\hat{y}}_i^t &= f_{dec}(\boldsymbol{z}_i^t)
\end{aligned}
      \label{eq:decoder}
\end{equation}


The reconstruction loss for model prediction is defined as the L2 distances between predicted trajectories to ground truth trajectories.

\begin{equation}
\mathcal{L}_{pred}=\sum_{i=1}^{N}\sum_{j=0}^{T}\left\|\boldsymbol{y}_i^{t_j}-\boldsymbol{\hat{y}}_i^{t_j}\right\|_2^2
\label{eq:lossReconstruct}
\end{equation}

\subsection{Time-Reversal Symmetry Constraints and Overall Training}
We additionally design a novel time-reversal symmetry loss as a soft constraint to flexibly regulate systems' total energy from changing sharply.
Specifically, based on the definition of time-reversal symmetry in Sec~\ref{sec:time_reversal}, we first conclude the following:


\begin{lemma}
\label{lemma:timereversal}   
Eq.\ref{eq:def_reverse} is equal to $R \circ \phi_t \circ R \circ \phi_t=id$, which implies that time-reversal symmetry is equivalent to the condition that trajectories can overlap when evolving backward from the final state.
\end{lemma}
This can be explained as the reversing of the forward time evolution of an arbitrary state should be equal to the backward time evolution of the reversed state.


We therefore first compute the reverse trajectories for each system by solving 

\begin{equation}
    \begin{aligned}
\dot{\boldsymbol{z}}_i^{r_t}:=\frac{d\boldsymbol{z}_i^{r_t}}{dt}=-g(\boldsymbol{z}_1^{r_t},\boldsymbol{z}_2^{r_t},\cdots \boldsymbol{z}_N^{r_t}), \quad \boldsymbol{z}_i^{r_{t_0}} = \boldsymbol{z}_i^T, \quad \boldsymbol{y}_i^{r_t} = f_{dec}(\boldsymbol{z}_i^{r_t})
    \end{aligned}
\end{equation}



Then the reversal loss is defined as the L2 distances between forward and reversed predictions.
\begin{equation}
    \label{eq:lossRODE}
\mathcal{L}_{reverse}=\sum_{i=1}^{N}\sum_{j=0}^{T}\left\|\boldsymbol{\hat{y}}_i^{t_j}-\boldsymbol{y}_i^{r_{T-j}}\right\|_2^2 
\end{equation}



Our time-reversal loss implementation is built upon Lemma\ref{lemma:timereversal} where our backward trajectories is starting from the last state of forward trajectories. One can also implement the loss by generating two backward trajectories starting from the same starting point similar as in~\cite{trsode}. However, we theoretically show that our implementation is guaranteed to have a lower error bound compared to the second method.


We next theoretically show that the time-reversal loss also numerically helps to reduce the prediction loss besides its physical meaning. Specifically, we show that it minimizes higher-order Taylor expansion terms during the ODE integration steps.



\begin{theorem} \label{thm: numerical}
% Let $\delta t$ denote the integration step size in an ODE solver and $\bm{z}_i=(q_i,p_i)$ be the state at timestamp $i$ with $q_i$ be the location and $p_i$ be the momentum which is related to velocity.
% When we do the forward evolution, the update function from timestamp $t_x$ to timestamp $t_y$ is  we evolve $\delta t$ from 
% state $\bm{z}_x=(p_x , q_x ,t_x)$ to the state $\bm{z}_{y}=(p_y , q_y , t_y)$, due toTaylor's Formula, the first-order momentum terms in $\delta t$ are nearly canceled out when computing the MSE between the forward and reverse evolutions in our loss function. This allows the neural network to focus on finer-scale optimizations.
% The original forward and ground truth prediction loss focus on minimizing the  first-order Taylor expansion terms during the ODE integration steps which related to the velocity and its scale is $\delta t$, and  time-reverse loss can help to focus on minimizing the  higher-order terms.


Let $\delta t$ denote the integration step size in an ODE solver and $T$ be the prediction length. The reconstruction loss defined in Eqn~\ref{eq:lossReconstruct} is  $\mathcal{O} (T^3 \delta t^2)$. The time-reversal loss defined in Eqn~\ref{eq:lossRODE} is $\mathcal{O} (T^5 \delta t^4)$. 

\end{theorem}
Theorem~\ref{thm: numerical} indicates that the time-reversal loss is forcing the model to predict fine-grained physical properties such as jerk (the derivatives of accelerations), compared with the reconstruction loss that forces the model to predict the locations/velocities accurately. Therefore, it enables our model to be more noise-tolerable. We prove Theorem~\ref{thm: numerical} in Appendix~\ref{appendix:proof_theoreom1}.



\textbf{Remark 1.}
% 1. justification of why choosing back-to-forward, instead of back-to-gt.
We define the reversal loss as the L2 distance between model forward trajectories and model backward trajectories. One can also choose to define the L2 distances between model backward trajectories and ground truth trajectories. However, it has two main drawbacks: (1) It does not naturally follow the time-reversal definition but instead uses an intermediate variable -- the ground truth trajectories to implicitly force such symmetry. (2) During the learning process, the forward trajectories may not be close to the ground truth in the very few epochs. Such implicit time-reversal implementation therefore would introduce more noise.

\textbf{Remark 2.} The time complexity brought by the reversal loss is linear to the forward predictions, as we use the ODE solver to fully predict the reverse trajectories just as the forward.
 The space complexity is only $\mathcal{O}(1)$ as we are using the adjoint methods to compute the reverse trajectories.

\begin{theorem} \label{thm: reverse traj}
    Comparing our method against the method following (\ref{eq:def_reverse}), 
    when the reconstruction loss (\ref{eq:lossReconstruct}) and the time-reversal loss (\ref{eq:lossRODE}) both have the same value between the two methods, our method achieves a smaller error $\max_{j \in [T]} \| \hat{\boldsymbol{y}} ^{t_j} - \boldsymbol{y} ^{r_{T - j}} \|_2$, which is the maximum distance between the reversal and ground truth trajectories. 
\end{theorem}
 Theorem~\ref{thm: reverse traj} suggests that our implementation of time-reversal symmetry is numerically better than the implementation used in~\cite{trsode}. We give the detailed proof in Appendix \ref{appendix:thm reverse traj}. 

Finally, we jointly train our model as a weighted combination of prediction loss and reversal loss as 
\begin{equation}
    \label{eq:overallLoss}
    \mathcal{L}=\mathcal{L}_{pred}+\alpha\mathcal{L}_{reverse}=\sum_{i=1}^{N}\sum_{j=0}^{T}\left\|\boldsymbol{y}_i^{t_j}-\boldsymbol{\hat{y}}_i^{t_j}\right\|_2^2
    +\alpha \sum_{i=1}^{N}\sum_{j=0}^{T}\left\|\boldsymbol{\hat{y}}_i^{t_j}-\boldsymbol{y}_i^{r_{T-j}}\right\|_2^2,
\end{equation}
where $\alpha$ is a positive coefficient to balance between the two losses based on different targeted systems.

% \WJ{TODO: multi agent loss proof using  inequality}
% \begin{lemma}
    
% \end{lemma}


==> section/relatedwork.tex <==
\section{Related Work}
\textbf{Neural Simulators for Multi-agent Dynamical Systems.}
Building a neural simulator that can understand and predict multi-agent system dynamics from observational data has attracted lots of attention.
Graph Neural Networks (GNNs) achieve the state-of-art performance which approximates pair-wise node (agent) interaction through message passing to impose strong spatial inductive bias. The majority of them are discrete models, which learn a fixed-step state transition function such as to predict trajectories from timestamp t to timestamp t+1. Despite their superior performance, discrete GNN models~\citep{IN,NRI,learn_to_simulate} have two main limitations: (1) they are not able to adequately model systems that are continuous in nature such as n-body systems. (2) they cannot deal with irregular-observed systems, where the observations for different agents are not temporally aligned and can happen at arbitrary time intervals. 
In contrast, neural ordinary differential equation (ODE) methods are continuous models that are superior to model system dynamics in the long-range and with irregular observations. Specifically, they employ GNN as the ODE function to model continuous system dynamics in the latent space,  with an encoder that infers latent initial states of nodes from historical data. These models are known as GraphODEs~\citep{LGODE,hope,ndcn}, which show superior generalization ability and efficiency in making long-range predictions.


\textbf{Physics-informed Neural Networks.}
Injecting physical inductive bias helps neural simulators to be trained more data efficiently and make more accurate predictions. Popular properties include 1.) \textit{Spatial Invariance}, \ie models should be invariant under geometric translation/rotation~\cite{e3gnn,keriven2019universal}; 2.) \textit{Energy conservation}~\cite{hamiltonianNN}, which preserves the total energies for the system over time. 
Towards the second category, not all systems are strictly energy-conservative. For non-isolated systems that have interactions with the environments, pure data-driven approaches may result in system energy changing sharply, which is unrealistic. We therefore would like to build a general-purpose model that can prevent such abrupt energy changes, so as to have the flexibility to cover both conservative and non-conservative dynamical systems.
One prior work also injects time-reversal symmetry into neural networks~\cite{trsode}. However, they cannot model multi-agent interactions and work only for fully-observable systems (with initial states as model input), while our method based on GraphODE is well suited for modelling multi-agent and irregularly observed system. We also theoretically connect time-reversal symmetry loss to how it helps to reduce numerical error. We also illustrate our implementation to achieve time-reversal symmetry has a lower error bound compared to their implementation. 







